Validity Learning on Failures: Mitigating the Distribution Shift in Autonomous Vehicle Planning

The planning problem constitutes a fundamental aspect of the autonomous driving framework. Recent strides in representation learning have empowered vehicles to comprehend their surrounding environments, thereby facilitating the integration of learning-based planning strategies. Among these approaches, Imitation Learning stands out due to its notable training efficiency. However, traditional Imitation Learning methodologies encounter challenges associated with the co-variate shift phenomenon. We propose Validity Learning on Failures, VL(on failure), as a remedy to address this issue. The essence of our method lies in deploying a pre-trained planner across diverse scenarios. Instances where the planner deviates from its immediate objectives, such as maintaining a safe distance from obstacles or adhering to traffic rules, are flagged as failures. The states corresponding to these failures are compiled into a new dataset, termed the failure dataset. Notably, the absence of expert annotations for this data precludes the applicability of standard imitation learning approaches. To facilitate learning from the closed-loop mistakes, we introduce the VL objective which aims to discern valid trajectories within the current environmental context. Experimental evaluations conducted on both reactive CARLA simulation and non-reactive log-replay simulations reveal substantial enhancements in closed-loop metrics such as \textit{Score, Progress}, and Success Rate, underscoring the effectiveness of the proposed methodology. Further evaluations against the Bench2Drive benchmark demonstrate that VL(on failure) outperforms the state-of-the-art methods by a large margin.

==> 4related_work.tex <==
\section{Related Work}

\noindent In this section, we present an overview of methods employed to address the planning problem. We categorize the existing approaches into two groups. The first category, known as Rule-based Optimization Planning, utilizes optimization and finite state machine systems for decision-making. These methods rely on predetermined costs and rewards that reflect desirable driving behavior and employ various optimization techniques to identify the most favorable solution \cite{IDM,ma2015efficient,zhang2022spatial,zhang2022sufficient}. Nonetheless, these methods encounter scalability issues due to the long-tail problem associated with corner cases and rare occurrences. This challenge becomes particularly pronounced in navigating complex urban driving scenarios, where defining cost functions can present difficulties. The second category, Learning-based Planning, leverages machine learning to estimate the optimal plan. Further subdivisions within learning-based planning include the following three groups:
\noindent\textbf{Reinforcement Learning (RL)} \cite{15sutton2018reinforcement} circumvents the intricacy of manually crafting diverse cost functions. Instead, RL relies on a reward signal to indicate desired behaviors. Deep RL employs neural networks to approximate the optimal policy that maximizes expected rewards. Nonetheless, practical RL training poses challenges due to safety and efficiency concerns in real-world environments \cite{16kendall2019learning}. Consequently, most methods utilize simulators and explicitly define reward signals \cite{17kiran2021deep,18shalev2016safe}. A significant limitation of RL methods is the manual design of simulators and reward functions \cite{19dosovitskiy2017carla,20lopez2018microscopic}, which restricts realism. Consequently, model transfer from simulation to reality may be constrained, hindering generalization to more complex urban scenarios \cite{21pan2017virtual,22osinski2020simulation,23amini2020learning}.
\noindent\textbf{Imitation Learning (IL)} originated in 1989 as a basic behavioral cloning method for rural road navigation \cite{26pomerleau1991efficient}. Subsequently, IL has been applied to highway driving \cite{27bojarski2016end} and urban environments \cite{28hawke2020urban}. However, behavioral cloning encounters challenges related to co-variate shift \cite{24ross2011reduction}. \cite{dart} propose an off-policy strategy that introduces noise into the supervisor's policy during demonstration collection. Similarly, \cite{bansal2019chauffeurnet} applies uniform perturbation to the vehicle's current pose and computes a new trajectory to return to the original target location. Nonetheless, rule-based trajectory augmentation methods may struggle to accurately capture the motion distribution influenced by the learner's policy, potentially leading to perturbed driving tendencies. This issue was addressed in limited highway and lane-following scenarios by framing the problem as a classification task \cite{29bojarski2020nvidia}. In parallel efforts, \cite{diffleMPC} and \cite{urban_driver} utilize a differentiable environment model, enabling actions to receive gradients from multiple future time steps and penalizing actions leading to significant future deviations. While \cite{diffleMPC} learns a data-driven dynamics model using a variational auto-encoder, \cite{urban_driver} develops a differentiable data-driven simulator to generate synthetic corrections to ego actions. However, the performance of these methods is contingent upon the accuracy of their simulator models. Adversarial Imitation Learning has been proposed to address this limitation \cite{31baram2017end,32ho2016generative}, but its application in autonomous vehicle planning remains limited, to the best of our knowledge.
\noindent\textbf{Inverse Reinforcement Learning (IRL)} leverages expert demonstrations to deduce the underlying reward function of the expert, which is subsequently utilized to train any standard RL algorithm. \cite{25ziebart2008maximum} employs the principle of maximum entropy to learn a reward function that maximizes the probability of expert trajectories while maintaining maximal uncertainty. This method offers greater flexibility in defining the reward function and can accommodate ambiguity in expert behavior. However, IRL may pose computational challenges and might not scale effectively to extensive state spaces. 
% Mid-representations and the availability of large-scale real-world AD datasets [6, 7] have been major enablers in recent years for tackling complex urban scenarios. Instead of learning policies directly from sensor data, the input of the model comprises the output of the perception system as well as an HD map of the area. 

% This representation compactly captures the nuance of urban scenarios and allows large-scale training on hundreds or thousands of hours of real driving situations. This led to new state-of-the-art solutions for motion forecasting [8, 9]. Moreover, [10] demonstrated that using mid-representations, large-scale datasets and simple behavioral cloning with perturbations [36] can scale and learn robust planning policies. The difficulty of this approach, however, is in engineering the noise model to overcome the covariate shift problem. Similar to URBAN-DRIVER, we use mid-level representations to build the simulator from real-world logs. This allows training in various realistic scenarios with other agents.







==> 6evaluation.tex <==
\section{Evaluation}
\begin{table*}[h]
    \centering
    \begin{tabular}{|c||c|c|c|c|c|}
         \hline
         & dataset & progress  & success & collision: back, front, side & ADBC \\
         \hline
         \hline
         IL & InD & 83.2$\pm$5.6 & 58.5$\pm$3.0 & 38.00$\pm$4.55: 9, 9.5, 19.5 & 147.53$\pm$19.03\\
         \hline
         IL + VL & InD & 84.1$\pm$3.4 & 61.3$\pm$2.5 & 36.00$\pm$2.55: 8.5, 10, 18.5 & 155.33$\pm$25.53\\
         \hline
         LfM-c & InD & 87.3$\pm$4.1& 65.33$\pm$6.11 & 25.33$\pm$2.89: 2.33, 6, 17 & 232.20$\pm$33.18\\
         \hline
         LfM-cs & InD & \textbf{98.7}$\pm$1.2 & \textbf{87}$\pm$0.0 & \textbf{10.00}$\pm$1.41: 2, 6, 2 & \textbf{600.37}$\pm$88.21\\
         \hline
    \end{tabular}
    \caption{ \small evaluation on InD}
    \label{tab:InD_closed_loop}
\end{table*}
\begin{table*}[h]
    \centering
    \begin{tabular}{|c||c|c|c|c|c|}
         \hline
         & dataset & overall-score  & ego-progress & no-collisions & TTCWB \\
         \hline
         \hline
         SimplePlanner & \makecell{Nuplan \\ (public testset)} & 0.294318 & 0.496391 & 0.732179 & 0.691446 \\
         \hline
         \makecell{UrbanDriver \\ (without augmentation)} & \makecell{Nuplan \\ (public testset)} & 0.388708 & 0.898438 & 0.639957 & 0.57265 \\
         \hline
         IDMPlanner & \makecell{Nuplan \\ (public testset)} & \textbf{0.702864 }& 0.837308 & \textbf{0.865385} & 0.752137\\
         \hline
         \makecell{IL \\ (our baseline)} & \makecell{Nuplan \\ (public testset)} & 0.373266 & 0.834959 & 0.614440 & 0.598545\\
         \hline
         LfM-cs & \makecell{Nuplan \\ (public testset)} & 0.665852 & \textbf{0.904197} & 0.812155 & \textbf{0.773481}\\
         \hline
    \end{tabular}
    \caption{ \small evaluation on Nuplan}
    \label{tab:nuplan_closed_loop}
\end{table*}
In this section we report our evaluation of the proposed algorithm and compare it against the state-of-the-art in the task of closed-loop planning. 
\subsection{Datasets}
We use two well known datasets, InD \cite{InD} and Nuplan \cite{nuplan}, for our training and evaluation on urban scenarios. The InD dataset is a new dataset of naturalistic vehicle trajectories recorded with the use of a drone at four different intersections. The Nuplan dataset is the world's first large-scale planning benchmark for autonomous driving.
\subsection{Evaluation metrics}
There are generally two category of metrics to evaluate a planner: 1- open-loop metrics that directly measure ego-forecasting accuracy using distance-based metrics, e.g FDE/ADE (final/average displacement errors) 2- closed-loop metrics that assess the long-term driving-relevant performance, e.g. progress, and collision rate. Similar to \cite{leader_board1}, we have also observed that improvements in open-loop metrics are not representative of the closed-loop performance. As a result, we only consider the closed-loop metrics. 

For evaluation on InD, we developed an efficient non-reactive data-replay simulator to compute the following closed-loop metrics:
\begin{itemize}
    \item progress along expert's route: average percent of the expert's route that the ego takes
    \item success rate: percent of the scenarios in which the ego can successfully reach the goal
    \item collision rate: percent of the scenarios in which the ego has a collision. We also report the side of the collision (front, back, or side).
    \item average distance between collisions (ADBC): total driving distance of the ego divided by the number of collisions
\end{itemize}

For further evaluation on NuPlan, we use the non-reactive closed-loop simulator and metrics provided in \cite{nuplan}. Specifically, we are interested in the following metrics:
\begin{itemize}
    \item progress along expert's route (ego-progress) : average percent of the expert's route that the ego takes
    \item no-ego-at-fault-collisions (no-collisions): percent of scenarios with no ego at fault collisions
    \item time-to-collision-within-bound (TTCWB): percent of scenarios in which minimum time to collision (TTC) during the scenario is larger than the predefined threshold (least-min-ttc = 0.95s)
\end{itemize}

\subsection{Baselines}

\noindent We compare our algorithm against the following baselines:
\begin{itemize}
    \item Imitation Learning (IL): the model described in section \ref{M1} which is trained with \textit{Imitation Learning} loss only. In other words, this baseline is equivalent to a standard \textit{Behavior Cloning} with a \textit{sample-based planner}. 
    \item Simple-Planner: a na\"{\i}ve planner that always plans a straight line with a constant speed.
    \item IDM \cite{IDM}: the Intelligent Driver Model (IDM) is a well-known model in the field of traffic flow theory and transportation engineering.
    \item Urban-Driver \cite{urban_driver}: an open-loop implementation of the urban-driver on Nuplan dataset. This baseline does not use any data augmenting methods.
\end{itemize}

\noindent Moreover, there can be various different rules to define the validity of a trajectory. We study and compare the effect of the two following validity checks:
\begin{itemize}
    \item \textit{Learning from Mistakes}, $invalid=\{ \text{collision}\}$ (\textit{LfM-c}): the valid set is the set of all candidates that don't have any collision in the planning horizon
    \item \textit{Learning from Mistakes}, $invalid=\{ \text{collision}, \text{stuck}\}$ (\textit{LfM-cs}): the valid set is the set of all candidates that don't have any collisions and are not stuck. More formally, a stuck trajectory is a trajectory that moves less than 1 meter when the ego has been stopped for the last two seconds and the road in its front is not blocked.
\end{itemize}

\subsection{Results}

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.55\linewidth}
        \includegraphics[width=\linewidth]{Figures/OpenloopIL1.png}
    \end{subfigure} 
    \caption{ \small effect of LfM on $l_{imitation}$: fine-tuning stage begins at iteration 100K leading to an extreme jump in the $l_{imitation}$. Colors stand for different seeds.} 
    \label{fig:LfM effect}
    \vspace{-10pt}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[t]{0.4\linewidth}
%         \includegraphics[width=\linewidth]{Figures/optimizingVL.png}
%         \caption{\small $l_{valid}$ when optimizing $l_{valid}+l_{imitation}$} (IL + VL)
%         \label{fig:optimVL}
%     \end{subfigure} \qquad
%     \begin{subfigure}[t]{0.4\linewidth}
%         \includegraphics[width=\linewidth]{Figures/not_optimizingVL.png}
%         \caption{\small $l_{valid}$ when optimizing $l_{imitation}$ only} (IL)
%         \label{fig:VL}    
%     \end{subfigure}
%     \caption{ \textit{Validity Learning} with open-loop data only}
%     \label{fig:no_optimVL}
%     \vspace{-10pt}
% \end{figure}

\noindent Table\ref{tab:InD_closed_loop} shows the closed-loop results on the InD dataset. The results suggests that \textit{LfM-cs} out performs the IL by a large margin. Our visual inspection of the model behavior shows that both \textit{LfM} models successfully learn to avoid collisions. However, the \textit{LfM-c} tends to get stuck in a safe zone and let the simulation time out. We also observed that many of the collision cases for \textit{LfM-c} are indirectly caused by getting stuck. While the ego is stuck in its safe zone, a non-reactive agent approaches the ego in a high speed. The ego tries to avoid the collision, but high speed of other agents combined with their non-reactive nature results in an inevitable collision. To avoid this issue, \textit{LfM-cs} uses a heuristic that marks the stuck behavior as invalid. As a result, the ego is always motivated to move whenever it can rather than to stop. 

\noindent We have further tested the \textit{LfM} performance on the Nuplan dataset. 
\noindent Table \ref{tab:nuplan_closed_loop} shows the closed-loop results on the Nuplan public testset. 
We observe that the performance of our IL only baseline is in par with the performance of the open-loop Urban Driver \cite{urban_driver} model. 
This observation matches our expectation as both models are simply two different implementations of the imitation learning idea. 
The \textit{LfM-cs} outperforms the imitation learning baselines in all the presented closed-loop metrics. 
The \textit{IDMPlanner} \cite{IDM} achieves a better overal-score, although \textit{LfM-cs} achieves a better progress score. 
It is important to highlight that, the IDMPlanner operates within the confines of a rule-based framework, which inherently limits its ability to scale effectively with increasing amounts of data, while LfM can further scale with data.


To deepen our comprehension of LfM's role in mitigating the distribution shift problem, we track the imitation loss $l_{imitation}$ (eq.\ref{eq:imitation_loss}) on open-loop expert data throughout the training process. Figure \ref{fig:LfM effect} illustrates the trend of $l_{imitation}$ during training. Notably, we observe a significant spike in the value of $l_{imitation}$ around iteration 100K, coinciding with the commencement of fine-tuning using closed-loop data (\textit{LfM}). Subsequent training leads to improvements in $l_{imitation}$; however, the values plateau at levels higher than the saturation levels observed before fine-tuning. We hypothesize that the lower saturation levels before fine-tuning compared to post-fine-tuning levels stem from overfitting. In essence, Validity Learning on closed-loop out-of-distribution data acts as a regularizer, curbing overfitting to in-distribution open-loop data.

\subsection{Ablation Study}

\noindent We conduct a detailed exploration of the effects of Validity Learning using solely open-loop data, without involving any closed-loop data collection. In our investigation of the influence of Validity Learning with open-loop data, we observe (without optimization) the value of the validity loss $l_{valid}$ while exclusively optimizing the imitation loss $l_{imitation}$. Fig.\ref{fig:no_optimVL} illustrates the values for validity loss ($l_{valid}$) during training when focusing solely on optimizing the imitation loss $l_{imitation}$. Remarkably, optimizing the imitation loss $l_{imitation}$ inherently leads to improvements in the validity loss $l_{valid}$. Furthermore, Fig.\ref{fig:optimVL} presents the values of the validity loss $l_{valid}$ during training when optimizing both the imitation loss $l_{imitation}$ and the validity loss $l_{valid}$. This experiment is denoted as IL+VL. Notably, optimizing the validity loss ($l_{valid}$) on open-loop data does not result in additional enhancements. The performance results in the closed-loop scenario corroborate this observation, as the performance difference between IL and IL+VL is statistically insignificant. In summary, Imitation Learning furnishes a more robust training signal compared to Validity Learning when utilizing open-loop data. Consequently, Validity Learning does not confer significant advantages in scenarios where expert annotation is available for open-loop data.

==> 6evaluation_include_Nuplan.tex <==
\section{Evaluation}
\begin{table*}[h]
    \centering
    \begin{tabular}{|c||c|c|c|c|c|}
         \hline
         & dataset & progress  & success & collision: back, front, side & ADBC \\
         \hline
         \hline
         
         \makecell{IL}  & InD & 83.2(5.6) & 58.5(3.0) & 38.00(4.55): 9,9.5,19.5 & 147.53(19.03)  \\
         \hline
         LFM-c  & InD & 87.3(4.1) & 65.33 (6.11) & 25.33(2.89):2.33,6,17 & 232.20(33.18)  \\
         \hline
         LFM-cs & InD & \textbf{98.7}(1.2) & \textbf{87} (0.0) & \textbf{10.00}(1.41):2,6,2 & \textbf{600.37} (88.21)  \\
         \hline
         \hline
         \makecell{IL}  & Nuplan & - & -  & - & -  \\
         \hline
         \makecell{LFM \\ ($valid=\{ \text{not collision}\}$)} & Nuplan & & & &  \\
         \hline
         \makecell{LFM \\ ($valid=\{ \text{not collision},$ \\$ \text{not stuck}\}$)} & Nuplan & & & &  \\
         \hline
    \end{tabular}
    \caption{ \small in-house closed-loop metrics}
    \label{tab:InD_closed_loop}
\end{table*}

\begin{table*}[h]
    \centering
    \begin{tabular}{|c||c|c|c|c|c|}
         \hline
         & data-set&overall-score & ego-progress-along-expert-route & no-ego-at-fault-collisions & time-to-collision-within-bound \\
         \hline
         \hline
         
         \makecell{UrbanDrive \\ (with augmentation) \cite{urban_driver}}  & \makecell{private testset \\ (leader board)}&0.6821 & 0.8417 & 0.8952 & 0.8065  \\
         \hline
         \makecell{IDMPlanner \cite{IDM}} & \makecell{private testset \\ (leader board)} & 0.7243 & 0.8144 & 0.8367 & 0.7762  \\
         \hline
         \makecell{CS-Tu \cite{leader_board1}} & \makecell{private testset \\ (leader board)}& 0.9276 & 0.9141 & 0.9879 & 0.9254 \\
         \hline
         \hline
         
         \makecell{SimplePlanner}  & public testset & 0.294318 & 0.496391 & 0.732179 & 0.691446 \\
         \hline
         \makecell{UrbanDrive \\ (without augmentation)}  &public testset & 0.388708  & 0.898438  & 0.639957 & 0.57265   \\
         \hline
         \makecell{IDMPlanner} & public testset & 0.702864 & 0.837308 & 0.865385 &  0.752137 \\
         \hline
         \makecell{IL}  & public testset & - & - & - & - \\
         \hline
         \makecell{LFM \\ ($valid=\{ \text{not collision}\}$)} & public testset & - & - & - & -  \\
         \hline
         \makecell{LFM \\ ($valid=\{ \text{not collision},$ \\$ \text{not stuck}\}$)} & public testset & - & - & - & -  \\
         \hline
    \end{tabular}
    \caption{ \small Nuplan closed-loop metrics}
    
    \label{tab:nuplan_closed_loop}
\end{table*}

In this section we report our evaluation of the proposed algorithm and compare it against the state-of-the-art in the task of closed-loop planning. 
\subsection{Datasets}
We use two well known datasets, InD \cite{InD} and Nuplan \cite{nuplan}, for our training and evaluation on urban scenarios. The InD dataset is a new dataset of naturalistic vehicle trajectories recorded with the use of a drone at four different intersections. The NuPlan dataset is the world's first large-scale planning benchmark for autonomous driving.
\subsection{Evaluation metrics}
There are generally two category of metrics to evaluate a planner: 1- open-loop metrics that directly measure ego-forecasting accuracy using distance-based metrics, e.g FDE/ADE (final/average displacement errors) 2- closed-loop metrics that assess the long-term driving-relevant performance, e.g. progress, and collision rate. Similar to \cite{leader_board1}, we have also observed that improvements in open-loop metrics are not representative of the closed-loop performance. As a result, we only consider the closed-loop metrics. 

For evaluation on InD, we developed an efficient non-reactive data-replay simulator to compute the following closed-loop metrics:
\begin{itemize}
    \item progress along expert's route: average percent of the expert's route that the ego takes
    \item success rate: percent of the scenarios in which the ego can successfully reach the goal
    \item collision rate: percent of the scenarios in which the ego has a collision. We also report the side of the collision (front, back, or side).
    \item average distance between collisions (ADBC): total driving distance of the ego divided by the number of collisions
\end{itemize}

For further evaluation on NuPlan, we use the non-reactive closed-loop simulator and metrics provided in \cite{nuplan}. Specifically, we are interested in the following metrics:
\begin{itemize}
    \item progress along expert's route: average percent of the expert's route that the ego takes
    \item no-ego-at-fault-collisions: percent of scenarios with no ego at fault collisions
    \item time-to-collision-within-bound: percent of scenarios in which minimum time to collision (TTC) during the scenario is larger than the predefined threshold (least-min-ttc = 0.95s)
\end{itemize}

\subsection{Baselines}

\noindent We compare our algorithm against the following baselines:
\begin{itemize}
    \item Imitation Learning (IL): a version of our model that is only trained with open-loop data imitation learning with a similar number of training steps.
    \item Simple-Planner: a na\"{\i}ve planner that always plans a straight line with a constant speed.
    \item IDM \cite{IDM}: the Intelligent Driver Model (IDM) on Nuplan dataset.
    \item Urban-Driver \cite{urban_driver}: an open-loop implementation of the urban-driver on Nuplan dataset
\end{itemize}

\noindent Moreover, there can be various different rules to define the validity of a trajectory. We study and compare the effect of the two following validity checks:
\begin{itemize}
    \item \textit{Learning from Mistakes}, $invalid=\{ \text{collision}\}$ (\textit{LfM-c}): the valid set is the set of all candidates that don't have any collision in the planning horizon
    \item \textit{Learning from Mistakes}, $invalid=\{ \text{collision}, \text{stuck}\}$ (\textit{LfM-cs}): the valid set is the set of all candidates that don't have any collisions and are not stuck. More formally, a stuck trajectory is a trajectory that moves less than 1 meter when the ego has been stopped for the last two seconds and the road in its front is not blocked.
\end{itemize}

\subsection{Results}

Table\ref{tab:InD_closed_loop} shows the closed-loop results on the InD dataset. The results suggests that \textit{LfM-cs} out performs the IL by a large margin. Our visual inspection of the model behavior shows that both \textit{LfM} models successfully learn to avoid collisions. However, the \textit{LfM-c} tends to get stuck in a safe zone and let the simulation to time out. We also observed that many of the collision cases for \textit{LfM-c} are also rooted in the stuck issue. While the ego is stuck in its safe zone, a non-reactive agent approaches the ego in a high speed. The ego tries to avoid the collision, but high speed of other agents combined with their non-reactive nature results in an inevitable collision. To avoid this issue, \textit{LfM-cs} uses a heuristic that marks the stuck behavior as invalid. As a result, the ego is always motivated to move whenever it can rather than to stop.  

To further evaluate our approach, we have tested the LFM algorithm on the Nuplan dataset. Table\ref{tab:nuplan_closed_loop} shows the closed-loop results on the Nuplan public test dataset. Note that 

==> links.tex <==
https://opendrivelab.com/e2ead/AD23Challenge/Track_4_AID.pdf

| score | ego_progress_along_expert_route | no_ego_at_fault_collisions | time_to_collision_within_bound | drivable_area_compliance | ego_is_comfortable |          |
|-------|---------------------------------|----------------------------|--------------------------------|--------------------------|--------------------|----------|
| 0.591681                        | 0.849587                   | 0.777778                       | 0.777778                 | 0.888889           | 0.833333 |
